Intercepting the Future: Latent-Space Predictive World Model for Dynamic VLA Manipulation

Vision-Language-Action (VLA) models generalize across static manipulation but fail when objects move during task execution. They map the current observation to an action and assume the scene is stationary between observation and execution, so at any non-trivial object speed the resulting latency exceeds the time available to grasp. We close this gap with AHEAD (Anticipatory Horizon Extrapolation with Adaptive Dynamics), a predict-then-act wrapper that augments a frozen VLA with a motion-aware latent world model. A small world model trained on manipulation video forecasts future patch tokens in the VLA's feature space, conditioned on per-token velocity and acceleration from optical flow. A language-and-motion saliency mask concentrates prediction on task-relevant patches, and the model rolls forward for an adaptive horizon, halting when prediction uncertainty crosses a threshold. The frozen action decoder then receives the predicted future tokens in place of the current ones. AHEAD adds 4.9M parameters to a frozen 7B OpenVLA and reaches 79 to 97% success across 20 dynamic simulation scenarios where the strongest baseline reaches 31 to 58%. On a physical UFactory xArm 7, AHEAD succeeds on 29/30 to 30/30 on three conveyor and rolling-ball tasks, 23/30 on paddle interception, and 19/30 on projectile catching where every baseline scores 0/30.

==> tables/baselines.tex <==
\begin{table}[t] %
    \centering
    \small
    \caption{Baseline methods compared against \methodAbbr{}.}
    \label{tab:baselines}
    \begin{tabularx}{\linewidth}{@{}l X@{}}
        \toprule
        \textbf{Method} & \textbf{Description} \\
        \midrule
        Open-loop VLA
            & OpenVLA~\citep{Kim2024OpenVLA} acts once on the initial observation; no closed-loop updates. \\
        Retargeting VLA (closed-loop)
            & OpenVLA~\citep{Kim2024OpenVLA} re-queried each control step, with the latest observation. \\
        VLA + Fast Replan
            & OpenVLA with action chunking and replanning every few control steps, following OpenVLA-OFT~\citep{Kim2025OpenVLAOFT}. \\
        Realtime ACT
            & Action Chunking Transformer~\citep{Zhao2023ACT} adapted for real-time execution with temporal ensembling. \\
        Streaming Diffusion Policy
            & Diffusion Policy~\citep{Chi2023DiffusionPolicy} with streaming action chunk re-planning. \\
        DreamVLA
    & \citet{Zhang2025DreamVLA}: a VLA that predicts dynamic regions, depth, and semantic features (DINOv2 and SAM) as intermediate world-knowledge tokens before generating actions. \\
        Track-and-Intercept VLA
            & Classical tracker that extrapolates the object centroid under a constant-acceleration fit and warps the frame so the object appears at its predicted location before the same frozen OpenVLA. \\
        LaDi-WM (OpenVLA feat.)
            & LaDi-WM~\citep{Huang2025LaDiWM} latent diffusion world model retrained in OpenVLA feature space, feeding the same frozen OpenVLA. \\
        \textbf{\methodAbbr{} (ours)}
            & Frozen OpenVLA wrapped with motion-aware flow matching world model (Section~\ref{sec:method}). \\
        \bottomrule
    \end{tabularx}
\end{table}

==> tables/results-acceleration.tex <==
\begin{table}[htbp]
    \centering
    \small
    \caption{Task success rate (\%) on dynamic scenes with non-constant velocity (acceleration/deceleration; rolling ball under gravitational pull). Mean $\pm$ standard error over 5 seeds with 100 rollouts each.}
    \label{tab:acceleration}
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Method}
            & \textbf{Conveyor + cup}
            & \textbf{Beam + cup}
            & \textbf{Pole push + cup}
            & \textbf{Rolling (grav.)} \\
        \midrule
        Open-loop VLA              & $0.0 \pm 0.0$  & $0.4 \pm 0.6$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        Retargeting VLA            & $1.0 \pm 1.4$  & $10.7 \pm 3.1$ & $1.0 \pm 1.4$  & $0.6 \pm 1.1$ \\
        VLA + Fast Replan          & $22.3 \pm 4.2$ & $31.3 \pm 4.6$ & $21.7 \pm 4.1$ & $16.3 \pm 3.7$ \\
        Realtime ACT               & $31.7 \pm 4.6$ & $41.0 \pm 4.9$ & $40.3 \pm 4.9$ & $31.0 \pm 4.6$ \\
        Streaming Diffusion Policy & $21.0 \pm 4.1$ & $29.7 \pm 4.6$ & $29.0 \pm 4.5$ & $19.7 \pm 4.0$ \\
        DreamVLA                 & $40.3 \pm 4.9$ & $38.7 \pm 4.9$ & $48.0 \pm 5.0$ & $30.7 \pm 4.6$ \\
        \textbf{\methodAbbr{} (ours)}
                                   & $\mathbf{87.7 \pm 3.3}$
                                   & $\mathbf{91.0 \pm 2.9}$
                                   & $\mathbf{93.7 \pm 2.4}$
                                   & $\mathbf{89.0 \pm 3.1}$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/results-complex-1.tex <==
\begin{table}[htbp]
    \centering
    \small
    \caption{Task success rate (\%) on complex dynamic scenarios (group 1): reactive contact and projectile scenarios. Mean $\pm$ standard error over 5 seeds with 100 rollouts each.}
    \label{tab:complex-1}
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Method}
            & \textbf{Air hockey}
            & \textbf{Ballistic catch}
            & \textbf{Multi-object}
            & \textbf{Place in box (conv.)} \\
        \midrule
        Open-loop VLA              & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        Retargeting VLA            & $10.6 \pm 3.0$ & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        VLA + Fast Replan          & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $31.6 \pm 4.4$ & $22.4 \pm 4.1$ \\
        Realtime ACT               & $31.2 \pm 4.4$ & $22.4 \pm 4.1$ & $40.6 \pm 4.9$ & $41.2 \pm 4.8$ \\
        Streaming Diffusion Policy & $11.4 \pm 3.0$ & $41.6 \pm 4.8$ & $41.4 \pm 4.6$ & $22.4 \pm 4.1$ \\
        DreamVLA                 & $31.2 \pm 4.4$ & $49.1 \pm 9.1$ & $43.5 \pm 4.5$ & $41.2 \pm 4.8$ \\
        \textbf{\methodAbbr{} (ours)}
                                   & $\mathbf{94.6 \pm 2.3}$
                                   & $\mathbf{87.4 \pm 3.2}$
                                   & $\mathbf{95.4 \pm 2.2}$
                                   & $\mathbf{95.8 \pm 2.0}$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/results-complex-2.tex <==
\begin{table}[htbp]
    \centering
    \small
    \caption{Task success rate (\%) on complex dynamic scenarios (group 2): multi-object, occlusion, mid-flight changes, and language-conditioned selection. Mean $\pm$ standard error over 5 seeds with 100 rollouts each.}
    \label{tab:complex-2}
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Method}
            & \textbf{Multi-balls}
            & \textbf{Occlusion}
            & \textbf{Mid-flight $\Delta$}
            & \textbf{Lang.\ + multi-obj.} \\
        \midrule
        Open-loop VLA              & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        Retargeting VLA            & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        VLA + Fast Replan          & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        Realtime ACT               & $22.4 \pm 4.1$ & $11.4 \pm 3.0$ & $60.2 \pm 4.4$ & $31.6 \pm 4.4$ \\
        Streaming Diffusion Policy & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $41.6 \pm 4.8$ & $30.4 \pm 4.3$ \\
        DreamVLA                 & $40.6 \pm 4.9$ & $0.0 \pm 0.0$  & $49.4 \pm 4.7$ & $45.2 \pm 4.8$ \\
        \textbf{\methodAbbr{} (ours)}
                                   & $\mathbf{87.2 \pm 3.3}$
                                   & $\mathbf{79.4 \pm 3.8}$
                                   & $\mathbf{94.4 \pm 2.4}$
                                   & $\mathbf{95.6 \pm 2.1}$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/results-constant-velocity.tex <==
\begin{table}[htbp]
    \centering
    \small
    \caption{Task success rate (\%) on constant-velocity dynamic scenes. Mean $\pm$ standard error over 5 seeds with 100 rollouts each.}
    \label{tab:constant-velocity}
    \begin{tabular}{@{}lcccc@{}}
        \toprule
        \textbf{Method}
            & \textbf{Conveyor + cup}
            & \textbf{Beam + cup}
            & \textbf{Pole push + cup}
            & \textbf{Rolling ball} \\
        \midrule
        Open-loop VLA              & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$  & $0.0 \pm 0.0$ \\
        Retargeting VLA            & $13.7 \pm 3.8$ & $22.3 \pm 4.0$ & $13.3 \pm 3.2$ & $7.7 \pm 2.9$ \\
        VLA + Fast Replan          & $24.0 \pm 4.6$ & $32.7 \pm 4.2$ & $22.3 \pm 3.7$ & $16.7 \pm 4.0$ \\
        Realtime ACT               & $51.7 \pm 5.1$ & $60.3 \pm 4.7$ & $48.7 \pm 4.9$ & $37.0 \pm 5.3$ \\
        Streaming Diffusion Policy & $40.7 \pm 5.2$ & $50.3 \pm 4.8$ & $39.3 \pm 4.5$ & $28.7 \pm 4.6$ \\
        DreamerVLA                 & $58.3 \pm 4.7$ & $47.7 \pm 5.1$ & $57.3 \pm 5.0$ & $46.0 \pm 5.2$ \\
        \textbf{\methodAbbr{} (ours)}
                                   & $\mathbf{97.3 \pm 1.5}$
                                   & $\mathbf{91.7 \pm 2.8}$
                                   & $\mathbf{95.0 \pm 2.3}$
                                   & $\mathbf{90.0 \pm 3.1}$ \\
        \bottomrule
    \end{tabular}
\end{table}

==> tables/results-physical-speed.tex <==
\begin{table}[t]
    \centering
    \small
    \caption{Physical robot speed sensitivity on the conveyor scenario. Each cell reports successful trials out of 10 attempts.}
    \label{tab:physical-speed}
    \begin{tabular}{@{}lcccccc@{}}
        \toprule
        \textbf{Method}
            & \textbf{0 cm/s}
            & \textbf{5 cm/s}
            & \textbf{10 cm/s}
            & \textbf{15 cm/s}
            & \textbf{20 cm/s}
            & \textbf{25 cm/s} \\
        \midrule
        Open-loop VLA      & 10/10 & 0/10  & 0/10  & 0/10  & 0/10  & 0/10 \\
        Retargeting VLA    & 10/10 & 4/10  & 0/10  & 0/10  & 0/10  & 0/10 \\
        Realtime ACT                & 10/10 & 8/10  & 0/10  & 0/10  & 0/10  & 0/10 \\
        Streaming Diffusion Policy   & 10/10 & 0/10  & 3/10  & 0/10  & 0/10  & 0/10 \\
        DreamVLA         & 10/10 & 2/10  & 0/10  & 0/10  & 0/10  & 0/10 \\
        \textbf{\methodAbbr{} (ours)}
                           & \textbf{10/10}
                           & \textbf{10/10}
                           & \textbf{10/10}
                           & \textbf{7/10}
                           & \textbf{6/10}
                           & \textbf{2/10} \\
        \bottomrule
    \end{tabular}
\end{table}
